Rescuing the End-user systems from Vulnerable Applications using Virtualization Techniques

In systems owned by normal end-users, many times security attacks are mounted by sneaking in malicious applications or exploiting existing software vulnerabilities through security non-conforming actions of users. Virtualization approaches can address this problem by providing a quarantine environment for applications, malicious devices, and device drivers, which are mostly used as entry points for security attacks. However, the existing methods to provide quarantine environments using virtualization are not transparent to the user, both in terms of application interface transparency and file system transparency. Further, software configuration level solutions like remote desktops and remote application access mechanisms combined with shared file systems do not meet the user transparency and security requirements. We propose qOS, a VM-based solution combined with certain OS extensions to meet the security requirements of end-point systems owned by normal users, in a transparent and efficient manner. We demonstrate the efficacy of qOS by empirically evaluating the prototype implementation in the Linux+KVM system in terms of efficiency, security, and user transparency.

==> arch.tex <==
\section{Architecture}
\label{sec:design}

\begin{figure}[tp]
 \centering
  \includegraphics[width=0.47\textwidth]{figures/design_alt.pdf}
  \caption{Architecture of qOS}
  \label{fig:design}
\end{figure}

The architecture of our system is given in Figure~\ref{fig:design}. 
The system consists of a virtual machine running inside the host system that we refer to as \textit{QuarantineVM} (or qVM). 
All the vulnerable applications are executed inside this qVM. 
%
\textit{AppLauncher} component performs application set up in the qVM 
at application execution time. The AppLauncher interacts with the \textit{Host OS Syscall Interceptor} to receive application initialization requests.  With qOS, the end-user is not entrusted to decide which applications are insecure and required to be executed in the quarantine. The AppLauncher concludes this based on verification from \textit{qSecurityMonitor}. %The AppLauncher also ensures that the application setup and launch in the qVM is automatic without having the user to interact with the qVM.

After the application is launched, the AppLauncher handles control to the \textit{HostEmbodiment} component, which acts as an encapsulation of the quarantine application and helps it to interact with the host system. This is required to maintain user transparency as the user must feel that the execution is on the host system.
%as who is waiting on the host system to provide a transparent application interface. 
Therefore, it facilitates quarantined applications to execute various file system and display related operations 
in the host system to provide a unified file system view to the user along with an experience of {\em local execution}. 
The HostEmbodiment is responsible for receiving requests from the application and executing them in the host system using the \textit{Host OS Syscall API}. %The HostEmbodiment should also be capable of running with multi-process applications like \textit{firefox}. The HostEmbodiment should act as the embodiment of all processes of an application.

The qSecurityMonitor mentioned earlier verifies whether an application is secure to run in the host system. 
For example, whenever the user tries to open a PDF file in a PDF viewer, 
the qSecurityMonitor checks if the PDF is verified and is not malicious. 
The qSecurityMonitor also has the responsibility of restricting the access of 
any files created by applications from qVM to the processes executing in the quarantine.
In other words, the qSecurityMonitor will never allow such 
a file to be opened or executed on the host system.

To facilitate communication between the host system and quarantine, the qOS consists of a \textit{Communication Channel} and a \textit{qChannelManager}. The qChannelManager, which is present on both host and qVM, is responsible for providing an interface for sending and receiving messages across both systems by using the Communication Channel. To meet the responsiveness requirements for applications running in qVM, 
the qChannelManager should be efficient and scalable.
%has significant stakes and needs to consider the following factors. 
Furthermore, qChannelManager should be capable of passing variable-sized messages over the channel.
%Furthermore, the qChannelManager should be efficient and scalable.
%in terms of utilizing the system resources. For example- CPU usage of the qChannelManager should not be significant.

Inside the host system, we have two more components---Host OS Syscall API and Host OS Syscall Interceptor. The Host OS Syscall API is responsible for providing the other host component with an interface to execute any system call in the host system. The Host OS Syscall Interceptor should be capable of intercepting and trapping any system call. The qVM also consists of similar components called \textit{Guest OS Syscall Interceptor} and \textit{Guest OS Syscall API}, which provides similar functionality.

Inside the qVM, we have a component called \textit{qDaemon}, which is responsible for launching the application inside the quarantine after receiving the launch request from AppLauncher through the Communication Channel. 

In the qOS design, it is needed that some system calls related to the filesystem and user interaction are routed to HostEmbodiment while remaining are performed in the qVM itself. To realize this, the qVM comprises of a component called \textit{SyscallRouter}. The SyscallRouter works with both qVM and host system and creates an abstraction of a singular base system for consistent execution of the quarantined application. The Guest OS Syscall Interceptor traps all the syscalls performed by the application and passes them to the SyscallRouter. The SyscallRouter is responsible for routing all these syscalls appropriately to different components. The SyscallRouter is also responsible for communicating necessary messages required to synchronize HostEmbodiment state. To increase the efficiency of application execution in qVM, the SyscallRouter should also limit communication with HostEmbodiment and avoid communication as much as possible.
%many requests in the quarantine itself. 

To illustrate the functioning of the architecture, let us consider the scenario where the user 
accidentally opens a malicious PDF in a PDF viewer application. 
The Host OS Syscall Interceptor catches the application launch request 
in the host system and passes it to the AppLauncher. 
The AppLauncher will consult the qSecurityMonitor to find that the PDF file is unverified and should be opened in the quarantine.
At this point, the AppLauncher will initiate application setup in 
qVM by communicating with the qDaemon, which will launch the PDF viewer in the qVM. 
The AppLauncher will then pass control to HostEmbodiment. 
Once the PDF viewer starts executing, all its system call will be trapped by the guest OS system call interceptor 
and moved to SyscallRouter. The SyscallRouter splits and routes the system calls such that the user still
interacts with the PDF viewer like a normal system.
%transfer all GUI system calls performed by the PDF viewer process to 
%the HostEmbodiment for creating PDF display and interacting with the user.
%taking user input and execute the remaining system call in qVM using Guest OS Syscall API. 
%The HostEmbodiment will perform all routed GUI syscalls in the host system. 
In this manner, the malicious PDF is opened in qVM to guarantee security with user transparency. 
Moreover, since the file is loaded from the host system itself, it provides a unified file system 
view to the end-user. 

